PCBEAR: Pose Concept Bottleneck for Explainable Action Recognition

Human action recognition (HAR) has achieved impressive results with deep learning models, but their decision-making process remains opaque due to their black-box nature. Ensuring interpretability is crucial, especially for real-world applications requiring transparency and accountability. Existing video XAI methods primarily rely on feature attribution or static textual concepts, both of which struggle to capture motion dynamics and temporal dependencies essential for action understanding. To address these challenges, we propose Pose Concept Bottleneck for Explainable Action Recognition (PCBEAR), a novel concept bottleneck framework that introduces human pose sequences as motion-aware, structured concepts for video action recognition. Unlike methods based on pixel-level features or static textual descriptions, PCBEAR leverages human skeleton poses, which focus solely on body movements, providing robust and interpretable explanations of motion dynamics. We define two types of pose-based concepts: static pose concepts for spatial configurations at individual frames, and dynamic pose concepts for motion patterns across multiple frames. To construct these concepts, PCBEAR applies clustering to video pose sequences, allowing for automatic discovery of meaningful concepts without manual annotation. We validate PCBEAR on KTH, Penn-Action, and HAA500, showing that it achieves high classification performance while offering interpretable, motion-driven explanations. Our method provides both strong predictive performance and human-understandable insights into the model's reasoning process, enabling test-time interventions for debugging and improving model behavior.

==> figure/experiments/acc.tex <==
\begin{figure*}[t]
% \figcapmargin
\includegraphics[width=\linewidth]{figure/img_files/ACC/ACC.png}

    \caption{\textbf{Performace.}}
    
    % \figcapmargin
\label{fig:acc}
\end{figure*}

==> figure/experiments/concept_contribution.tex <==
\begin{figure}
    \centering
    \subfigure[]{
        \includegraphics[widht=0.5\linewidth]{figure/img_files/experiments/concept contribution/concept_contribution_penn.pdf}
        \caption{Penn Action "Jumping jack"}
        \label{fig:cc_jumpingjack}
    }
    \centering
    \subfigure[]{
        \includegraphics[widht=0.5\linewidth]{figure/img_files/experiments/concept contribution/concept_contribution_walking.pdf}
        \caption{KTH-5 "walking"}
        \label{fig:cc_walking}
    }
\end{figure}

==> figure/experiments/static_check.tex <==
\begin{figure}[t]
% \figcapmargin
\includegraphics[width=0.9\linewidth]{figure/img_files/experiments/static/temp.pdf}
    \centering
    \captionsetup{justification=justified, singlelinecheck=false}
    \caption{\textbf{Evaluation of temporal learning using static frames. } The figure illustrates an experiment where a single frame from the test video is extracted and used to construct a new test input. }
    % \figcapmargin
\label{fig:static_check}
\end{figure}

==> figure/experiments/task_level.tex <==
\begin{figure*}[t]
% \figcapmargin
\includegraphics[width=10cm]{figure/img_files/group_level/group_level.pdf}
    \captionsetup{justification=justified, singlelinecheck=false}
    \caption{\textbf{Visualization of task-level concept contributions for the Penn Action dataset. } The figure illustrates the most dominant concepts utilized across various action classes, highlighting the key motion patterns that the model frequently relies on.}
    % \figcapmargin
\label{fig:task_level}
\end{figure*}

==> figure/fig_motivation.tex <==
\begin{figure*}[t]
    \centering
    \captionsetup{justification=justified, singlelinecheck=false}
    \includegraphics[width=0.8\linewidth]
    {figure/img_files/concept.pdf}
    \caption{\textbf{Concept Preprocessing Overview.}
    (a) Given video frames, we extract three concept types—Object Context, Action Context, and Scene Context—using LLaVA with carefully designed prompts. The extracted concepts are filtered and organized into Object, Action, and Scene concept sets. Our video CBM leverages these concept sets to train concept layers for the three attributes.
    (b) To reduce the cost of concept labeling, we adopt a label-free approach~\cite{lf-cbm}. Given a concept set, we pass input videos and the concept set through a video-text multi-modal encoder to obtain video feature vectors and text feature vectors. By computing the inner product of these feature vectors, we construct a concept matrix, which indicates the similarity between each video and the concepts. This concept matrix serves as pseudo-labels for training the concept layers. For instance, the red box highlights the vector containing the soft labels of each concept for  $v_1$.}
    \label{fig:concept}
    \vspace{-0.5em}
\end{figure*}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> table/accuracy.tex <==
\begin{table}[t]
\centering
\captionsetup{justification=justified, singlelinecheck=false}
\caption{{VideoCBM achieve comparable performance to the original models on UCF101, Kinetics400 and SSV2.} We evaluate the performance of the video action recognition models across different video datasets} 
% \vspace{\tabcapmargin}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{Top-1 Accuracy.} \\
\cmidrule(lr) {2-4}
Model &  UCF101 & Kinetics400& SSV2  \\
\midrule
AIM & 93.1  & 71.3 & 61.5\\
VideoMAE & 92.5  & 70.5& 65.5 \\
\midrule
AIM(V-CBM) & 98.1 & 68.0 & 58.3 \\
VideoMAE(V-CBM) & 98.4 & 67.7 & 62.8 \\
\bottomrule
\end{tabular}
}
\label{tab:comparison}
\end{table}
